Deep Learning Approaches to Quantum Error Mitigation

We present a systematic investigation of deep learning methods applied to quantum error mitigation of noisy output probability distributions from measured quantum circuits. We compare different architectures, from fully connected neural networks to transformers, and we test different design/training modalities, identifying sequence-to-sequence, attention-based models as the most effective on our datasets. These models consistently produce mitigated distributions that are closer to the ideal outputs when tested on both simulated and real device data obtained from IBM superconducting quantum processing units (QPU) up to five qubits. Across several different circuit depths, our approach outperforms other baseline error mitigation techniques. We perform a series of ablation studies to examine: how different input features (circuit, device properties, noisy output statistics) affect performance; cross-dataset generalization across circuit families; and transfer learning to a different IBM QPU. We observe that generalization performance across similar devices with the same architecture works effectively, without needing to fully retrain models.

==> TABLES_final/cross-testing-alternative.tex <==
% Preamble additions (do once):
% \usepackage{needspace}
% \usepackage{booktabs,longtable,multirow,array}
% \usepackage[dvipsnames]{xcolor}

{\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.9}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}

\begin{longtable}{@{\extracolsep{\fill}}>{\raggedright\arraybackslash}m{2.9cm}lcccc@{}}
\label{tab:cross_testing_l1_results}\\

\toprule
Dataset & Model & L1RC Median ($\pm$SE) & P25 & P75 & L1RC \% Improved \\
\midrule
\endfirsthead

\toprule
Dataset & Model & L1RC Median ($\pm$SE) & P25 & P75 & L1RC \% Improved \\
\midrule
\endhead

\bottomrule
\endfoot

\bottomrule
\caption{Standard vs Cross testing for L1 Relative Change. The table reports the median ($\pm$SE) and interquartile range (P25--P75) of the L1 relative change across datasets, with the final column showing the percentage of circuits that are improved, as compared to the noisy baseline. In \textbf{bold} the best performing model per dataset, in green improvements over the noisy baseline, in red worse results than the baseline.}\\
\endlastfoot

% ===================== SIMULATED SECTION =====================
\multicolumn{6}{l}{\textbf{Simulated}}\\
\midrule

\Needspace{12\baselineskip}
\multirow[t]{8}{2.9cm}{\raggedright Algiers Pauli Simulated (Standard)}
 & MLP            & \textcolor{BrickRed}{0.2047 $\pm$ 0.0010} & \textcolor{BrickRed}{0.0006} & \textcolor{BrickRed}{0.5333} & 24.4\% \\
 & MLP\text{-}PRED& \textcolor{ForestGreen}{-0.0935 $\pm$ 0.0008} & \textcolor{ForestGreen}{-0.2884} & \textcolor{BrickRed}{0.1045} & 62.3\% \\
 & ENC            & \textcolor{BrickRed}{0.2041 $\pm$ 0.0010} & \textcolor{BrickRed}{0.0012} & \textcolor{BrickRed}{0.5296} & 23.9\% \\
 & RNN            & \textcolor{ForestGreen}{-0.4935 $\pm$ 0.0006} & \textcolor{ForestGreen}{-0.6330} & \textcolor{ForestGreen}{-0.2681} & 90.4\% \\
 & \textbf{TF}    & \textcolor{ForestGreen}{-0.6326 $\pm$ 0.0004} & \textcolor{ForestGreen}{-0.7295} & \textcolor{ForestGreen}{-0.4645} & 94.0\% \\
 & TFM            & \textcolor{ForestGreen}{-0.6254 $\pm$ 0.0004} & \textcolor{ForestGreen}{-0.7239} & \textcolor{ForestGreen}{-0.4577} & 94.0\% \\
 & NOISY\text{-}ENC & \textcolor{ForestGreen}{-0.6248 $\pm$ 0.0005} & \textcolor{ForestGreen}{-0.7304} & \textcolor{ForestGreen}{-0.4328} & 92.9\% \\
 & PERCEIVER      & \textcolor{ForestGreen}{-0.5727 $\pm$ 0.0006} & \textcolor{ForestGreen}{-0.7052} & \textcolor{ForestGreen}{-0.3458} & 91.0\% \\
\midrule

\Needspace{12\baselineskip}
\multirow[t]{8}{2.9cm}{\raggedright Train Random Sim $\rightarrow$ Test Pauli Sim (Cross)}
 & MLP            & \textcolor{BrickRed}{0.4115 $\pm$ 0.0024} & \textcolor{ForestGreen}{-0.0015} & \textcolor{BrickRed}{1.0440} & 26.8\% \\
 & MLP\text{-}PRED& \textcolor{BrickRed}{0.3596 $\pm$ 0.0015} & \textcolor{BrickRed}{0.0172} & \textcolor{BrickRed}{0.9375} & 22.2\% \\
 & ENC            & \textcolor{BrickRed}{0.1770 $\pm$ 0.0010} & \textcolor{ForestGreen}{-0.0011} & \textcolor{BrickRed}{0.6146} & 26.2\% \\
 & RNN            & \textcolor{BrickRed}{0.3693 $\pm$ 0.0023} & \textcolor{ForestGreen}{-0.0232} & \textcolor{BrickRed}{1.0173} & 29.2\% \\
 & TF             & \textcolor{ForestGreen}{-0.4589 $\pm$ 0.0006} & \textcolor{ForestGreen}{-0.5819} & \textcolor{ForestGreen}{-0.2208} & 88.7\% \\
 & \textbf{TFM}   & \textcolor{ForestGreen}{-0.5217 $\pm$ 0.0004} & \textcolor{ForestGreen}{-0.6221} & \textcolor{ForestGreen}{-0.3602} & 93.9\% \\
 & NOISY\text{-}ENC & \textcolor{ForestGreen}{-0.5055 $\pm$ 0.0005} & \textcolor{ForestGreen}{-0.6183} & \textcolor{ForestGreen}{-0.3375} & 94.3\% \\
 & PERCEIVER      & \textcolor{ForestGreen}{-0.0610 $\pm$ 0.0008} & \textcolor{ForestGreen}{-0.2509} & \textcolor{BrickRed}{0.0960} & 60.6\% \\
\addlinespace[0.6mm]

\Needspace{12\baselineskip}
\multirow[t]{8}{2.9cm}{\raggedright Algiers Random Simulated (Standard)}
 & MLP            & \textcolor{ForestGreen}{-0.0753 $\pm$ 0.0007} & \textcolor{ForestGreen}{-0.2399} & \textcolor{BrickRed}{0.1038} & 62.9\% \\
 & MLP\text{-}PRED& \textcolor{BrickRed}{0.3961 $\pm$ 0.0011} & \textcolor{BrickRed}{0.1370} & \textcolor{BrickRed}{0.7509} & 11.8\% \\
 & ENC            & \textcolor{BrickRed}{0.2765 $\pm$ 0.0007} & \textcolor{BrickRed}{0.1340} & \textcolor{BrickRed}{0.5161} & 9.5\% \\
 & RNN            & \textcolor{ForestGreen}{-0.0650 $\pm$ 0.0004} & \textcolor{ForestGreen}{-0.1697} & \textcolor{BrickRed}{0.0399} & 67.4\% \\
 & TF             & \textcolor{ForestGreen}{-0.5288 $\pm$ 0.0005} & \textcolor{ForestGreen}{-0.6435} & \textcolor{ForestGreen}{-0.3039} & 89.4\% \\
 & TFM            & \textcolor{ForestGreen}{-0.5230 $\pm$ 0.0005} & \textcolor{ForestGreen}{-0.6381} & \textcolor{ForestGreen}{-0.2956} & 89.2\% \\
 & NOISY\text{-}ENC & \textcolor{ForestGreen}{-0.4740 $\pm$ 0.0006} & \textcolor{ForestGreen}{-0.6022} & \textcolor{ForestGreen}{-0.1900} & 84.7\% \\
 & \textbf{PERCEIVER} & \textcolor{ForestGreen}{-0.5453 $\pm$ 0.0004} & \textcolor{ForestGreen}{-0.6446} & \textcolor{ForestGreen}{-0.3613} & 91.7\% \\
\midrule

\Needspace{12\baselineskip}
\multirow[t]{8}{2.9cm}{\raggedright Train Pauli Sim $\rightarrow$ Test Random Sim (Cross)}
 & MLP            & \textcolor{BrickRed}{0.6421 $\pm$ 0.0014} & \textcolor{BrickRed}{0.3016} & \textcolor{BrickRed}{1.2221} & 6.0\% \\
 & MLP\text{-}PRED& \textcolor{BrickRed}{1.0722 $\pm$ 0.0021} & \textcolor{BrickRed}{0.5587} & \textcolor{BrickRed}{1.8176} & 3.4\% \\
 & ENC            & \textcolor{BrickRed}{0.4898 $\pm$ 0.0017} & \textcolor{BrickRed}{0.1456} & \textcolor{BrickRed}{1.1084} & 8.5\% \\
 & RNN            & \textcolor{ForestGreen}{-0.1626 $\pm$ 0.0012} & \textcolor{ForestGreen}{-0.3899} & \textcolor{BrickRed}{0.1401} & 64.1\% \\
 & TF             & \textcolor{ForestGreen}{-0.1902 $\pm$ 0.0013} & \textcolor{ForestGreen}{-0.4588} & \textcolor{BrickRed}{0.1888} & 63.4\% \\
 & \textbf{TFM}   & \textcolor{ForestGreen}{-0.2004 $\pm$ 0.0013} & \textcolor{ForestGreen}{-0.4601} & \textcolor{BrickRed}{0.1699} & 64.1\% \\
 & NOISY\text{-}ENC & \textcolor{ForestGreen}{-0.1119 $\pm$ 0.0015} & \textcolor{ForestGreen}{-0.4162} & \textcolor{BrickRed}{0.3005} & 58.6\% \\
 & PERCEIVER      & \textcolor{BrickRed}{0.0704 $\pm$ 0.0011} & \textcolor{ForestGreen}{-0.1582} & \textcolor{BrickRed}{0.6600} & 41.6\% \\
\addlinespace[0.6mm]

% ===================== REAL SECTION =====================
\multicolumn{6}{l}{\textbf{Real}}\\
\midrule

\Needspace{12\baselineskip}
\multirow[t]{8}{2.9cm}{\raggedright Algiers Pauli Real (Standard)}
 & MLP            & \textcolor{ForestGreen}{-0.0238 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.1812} & \textcolor{BrickRed}{0.0128} & 64.5\% \\
 & MLP\text{-}PRED& \textcolor{ForestGreen}{-0.1176 $\pm$ 0.0005} & \textcolor{ForestGreen}{-0.3142} & \textcolor{BrickRed}{0.0140} & 71.9\% \\
 & ENC            & \textcolor{ForestGreen}{-0.0155 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.1723} & \textcolor{BrickRed}{0.0276} & 58.6\% \\
 & RNN            & \textcolor{ForestGreen}{-0.1891 $\pm$ 0.0006} & \textcolor{ForestGreen}{-0.4060} & \textcolor{ForestGreen}{-0.0298} & 81.2\% \\
 & \textbf{TF}    & \textcolor{ForestGreen}{-0.2039 $\pm$ 0.0007} & \textcolor{ForestGreen}{-0.4471} & \textcolor{ForestGreen}{-0.0324} & 82.5\% \\
 & TFM            & \textcolor{ForestGreen}{-0.2027 $\pm$ 0.0007} & \textcolor{ForestGreen}{-0.4460} & \textcolor{ForestGreen}{-0.0320} & 82.5\% \\
 & NOISY\text{-}ENC & \textcolor{ForestGreen}{-0.1910 $\pm$ 0.0006} & \textcolor{ForestGreen}{-0.4335} & \textcolor{ForestGreen}{-0.0293} & 81.6\% \\
 & PERCEIVER      & \textcolor{ForestGreen}{-0.2033 $\pm$ 0.0006} & \textcolor{ForestGreen}{-0.4533} & \textcolor{ForestGreen}{-0.0326} & 82.9\% \\
\midrule

\Needspace{12\baselineskip}
\multirow[t]{8}{2.9cm}{\raggedright FT Random Real $\rightarrow$ Test Pauli Real (Cross)}
 & MLP            & \textcolor{ForestGreen}{-0.0165 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.1994} & \textcolor{BrickRed}{0.0203} & 60.4\% \\
 & MLP\text{-}PRED& \textcolor{ForestGreen}{-0.0299 $\pm$ 0.0003} & \textcolor{ForestGreen}{-0.2137} & \textcolor{BrickRed}{0.0527} & 59.0\% \\
 & ENC            & \textcolor{BrickRed}{0.0110 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.0720} & \textcolor{BrickRed}{0.0456} & 41.4\% \\
 & RNN            & \textcolor{ForestGreen}{-0.0211 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.1951} & \textcolor{BrickRed}{0.0094} & 65.1\% \\
 & \textbf{TF}    & \textcolor{ForestGreen}{-0.0405 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.1642} & \textcolor{BrickRed}{0.0026} & 72.6\% \\
 & TFM            & \textcolor{ForestGreen}{-0.0341 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.1506} & \textcolor{BrickRed}{0.0049} & 70.5\% \\
 & NOISY\text{-}ENC & \textcolor{ForestGreen}{-0.0261 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.1361} & \textcolor{BrickRed}{0.0131} & 65.0\% \\
 & PERCEIVER      & \textcolor{ForestGreen}{-0.0325 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.1260} & \textcolor{BrickRed}{0.0046} & 70.8\% \\
\addlinespace[0.6mm]

\Needspace{12\baselineskip}
\multirow[t]{8}{2.9cm}{\raggedright Algiers Random Real (Standard)}
 & MLP            & \textcolor{BrickRed}{0.0066 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.0178} & \textcolor{BrickRed}{0.0606} & 42.4\% \\
 & MLP\text{-}PRED& \textcolor{BrickRed}{0.0866 $\pm$ 0.0003} & \textcolor{BrickRed}{0.0106} & \textcolor{BrickRed}{0.1944} & 21.8\% \\
 & ENC            & \textcolor{BrickRed}{0.0162 $\pm$ 0.0002} & \textcolor{ForestGreen}{-0.0245} & \textcolor{BrickRed}{0.1078} & 39.9\% \\
 & RNN            & \textcolor{BrickRed}{0.0060 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.0175} & \textcolor{BrickRed}{0.0463} & 43.1\% \\
 & TF             & \textcolor{ForestGreen}{-0.0166 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.0812} & \textcolor{BrickRed}{0.0162} & 63.0\% \\
 & TFM            & \textcolor{ForestGreen}{-0.0168 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.0822} & \textcolor{BrickRed}{0.0169} & 62.8\% \\
 & NOISY\text{-}ENC & \textcolor{ForestGreen}{-0.0182 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.0929} & \textcolor{BrickRed}{0.0207} & 62.2\% \\
 & \textbf{PERCEIVER} & \textcolor{ForestGreen}{-0.0210 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.1013} & \textcolor{BrickRed}{0.0156} & 64.6\% \\
\midrule

\Needspace{12\baselineskip}
\multirow[t]{8}{2.9cm}{\raggedright FT Pauli Real $\rightarrow$ Test Random Real (Cross)}
 & MLP            & \textcolor{BrickRed}{0.0127 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.0170} & \textcolor{BrickRed}{0.1115} & 38.9\% \\
 & MLP\text{-}PRED& \textcolor{BrickRed}{0.3684 $\pm$ 0.0007} & \textcolor{BrickRed}{0.1618} & \textcolor{BrickRed}{0.6454} & 9.7\% \\
 & \textbf{ENC}   & \textcolor{BrickRed}{0.0116 $\pm$ 0.0001} & \textcolor{ForestGreen}{-0.0216} & \textcolor{BrickRed}{0.0732} & 40.6\% \\
 & RNN            & \textcolor{BrickRed}{0.0809 $\pm$ 0.0003} & \textcolor{ForestGreen}{-0.0218} & \textcolor{BrickRed}{0.2532} & 29.8\% \\
 & TF             & \textcolor{BrickRed}{0.0478 $\pm$ 0.0003} & \textcolor{ForestGreen}{-0.0341} & \textcolor{BrickRed}{0.2178} & 34.4\% \\
 & TFM            & \textcolor{BrickRed}{0.0453 $\pm$ 0.0003} & \textcolor{ForestGreen}{-0.0345} & \textcolor{BrickRed}{0.2116} & 34.6\% \\
 & NOISY\text{-}ENC & \textcolor{BrickRed}{0.0634 $\pm$ 0.0003} & \textcolor{ForestGreen}{-0.0264} & \textcolor{BrickRed}{0.2341} & 31.8\% \\
 & PERCEIVER      & \textcolor{BrickRed}{0.0442 $\pm$ 0.0003} & \textcolor{ForestGreen}{-0.0315} & \textcolor{BrickRed}{0.2079} & 34.4\% \\

\end{longtable}
}

==> preamble.tex <==
%
% LaTeX2e Preamble / Ross Duncan 2011
%
%-------------------------------------------------------
% TODO 27/1/2011
% 1. Something for tikz
% 2. Font alternatives?
% 3. Which journals clash with which bits?
% 4. No support for logic -- proof trees linear logic symbols etc
% 5. Use switches to turn on/off some parts
%-------------------------------------------------------

% typographical improvements
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{microtype}
%\usepackage[stretch=10]{microtype} % more conservative
%\usepackage[expansion=false]{microtype} % still more conservative
\usepackage{xspace}
\usepackage{enumitem}
\usepackage{amsmath}  % for \text
\usepackage{multirow} % for multi-row cells
\usepackage{booktabs} % for improved table formatting
\usepackage{url}
\usepackage{float}

% make figs a bit nicer
\newcommand{\figureline}{\rule{\textwidth}{0.5pt}}
\newcommand{\figureend}{\rule{\textwidth}{0.5pt}}

% do The Right Thing
\makeatletter
\newcommand\etc{etc\@ifnextchar.{}{.\@}\xspace}
\newcommand\ie{i.e.\@\xspace}  % these two may be broken
\newcommand\eg{e.g.\@\xspace}
\makeatother

% arg is height; optional arg is baseline shift
\newcommand{\vstrut}[2][0pt]{\rule[#1]{0pt}{#2}}

% including code bits
\newcommand{\code}[1]{\vspace{1ex} \par \parindent=1.3cm \hangindent=1.5cm
                           \texttt{\small #1 \normalsize} \vspace{1ex}
                           \parindent=15pt \par\noindent}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Include graphics in a nice way
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{graphicx}
\usepackage{needspace}
%%%% Use these commands to insert graphics into
%%%% the text and have them line up properly.

%%% - inlinegraphic requires absolute size to be given
%%% - ninlinegraphic uses optional scaling factor

%%%% first param is the desired height of the graphic
%%%% if it is less the 1ex, it might not look good
\newcommand{\inlinegraphic}[2]{
  %% todo -- make this thing calculate the height
  %% itself based on a global scaling factor
  \dimendef\grafheight=255\dimendef\grafvshift=254
  \grafheight=#1
  \grafvshift=-0.5\grafheight
  \advance\grafvshift by 0.5ex
  \raisebox{\grafvshift}{\includegraphics[height=\grafheight]{images/#2}\xspace}
}


%%% optional first arg is scaling factor
\newcommand{\ninlinegraphic}[2][1.0]{
  \dimendef\grafheight=255\dimendef\grafvshift=254
  \setbox0 = \hbox{\scalebox{#1}{\includegraphics{images/#2}}}
  \grafheight=\the\ht0
  \grafvshift=-0.5\grafheight
  \advance\grafvshift by 0.5ex
  \raisebox{\grafvshift}{\includegraphics[height=\grafheight]{images/#2}\xspace}
}

\newcommand{\inline}[1]{
  \raisebox{0.5ex}{\;#1\;}
}

%%%%%%%%%%%
% text colours
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\red}[1]{{\color{red}#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Mathematical packages and theorems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{amsmath} % can collide with some journals
\usepackage{stmaryrd}
\usepackage{mathtools}
\usepackage{stackrel}
%%% not needed if amsmath loaded
% \newcommand{\text}[1]{\ensuremath{\mbox{#1}}}


%%% Defining theorems and friends usually makes problems for journal
%%% styles
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}\newtheorem{example}[theorem]{Example}
\theoremstyle{definition}\newtheorem{examples}[theorem]{Examples}
\theoremstyle{definition}\newtheorem{definition}[theorem]{Definition}
\theoremstyle{definition}\newtheorem{definitions}[theorem]{Definitions}
\theoremstyle{definition}\newtheorem{remark}[theorem]{Remark}
\theoremstyle{definition}\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{notation}[theorem]{Notation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General Mathematics shorthands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% aliases
\newcommand{\infinity}{\infty}
\newcommand{\iso}{\cong}
\newcommand{\isomorphism}{\cong}
\newcommand{\vd}{\ensuremath{\vdash}}  % = turnstyle

\newcommand{\dom}{\operatorname{dom}}
\newcommand{\cod}{\operatorname{cod}}
\newcommand{\Tr}{\operatorname{Tr}}

\newcommand{\denote}[1]{% --``semantic'' brakets
\llbracket #1 \rrbracket}
\newcommand{\ldenote}[1]{\left\llbracket #1 \right\rrbracket}
\newcommand{\name}[1]{%---  name / coname
\ulcorner #1 \urcorner}
\newcommand{\coname}[1]{%
\llcorner #1 \lrcorner}
\newcommand{\sizeof}[1]{% \sizeof{x} == |x|
  \left|#1\right|}

% ot is to backwards
\newcommand{\ot}{\leftarrow}
% for partial functions
\newcommand{\harto}{\rightharpoonup}


\newcommand{\NN}{\ensuremath{\mathbb{N}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Quantum Notations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bra}[1]{%  dirac 'bra'
    \ensuremath{\left\langle #1 \right|}\xspace}
\newcommand{\ket}[1]{%  dirac 'ket'
    \ensuremath{\left|  #1 \right\rangle}\xspace}
\newcommand{\innp}[2]{%  dirac style inner product
    \ensuremath{\langle #1 \mid #2 \rangle}}
\newcommand{\outp}[2]{%  dirac style outer product
    \ensuremath{\left|\left. #1 \rangle\right.\langle\left. #2 \right|\right. }}
\newcommand{\norm}[1]{% define command to get spacing right
        \ensuremath{\left| #1 \right| }}

% aliases for circuits
\newcommand{\CZ}{\ensuremath{\wedge Z}\xspace}
\newcommand{\CX}{\ensuremath{\wedge X}\xspace}
\newcommand{\CNot}{\CX}

\newcommand{\CNOT}{\ensuremath{\textsc{cnot}}\xspace}
\newcommand{\TONC}{\ensuremath{\textsc{tonc}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time to define some category  theory stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Objects of ???
\newcommand{\OBJ}[1]{\ensuremath{\mathrm{Obj}_{#1}}}
% Objects of {\cal ??}
\newcommand{\OBJC}[1]{\ensuremath{\mathrm{Obj}_{{\cal #1}}}}
% Arrows of ???
\newcommand{\ARR}[1]{\ensuremath{\mathrm{Arr}_{#1}}}
% Arrows of {\cal ??}
\newcommand{\ARRC}[1]{\ensuremath{\mathrm{Arr}_{{\cal #1}}}}

% sub scripted identity morphisms
\ifx\numericids\undefined
\newcommand{\id}[1]{\ensuremath{\mathrm{id}_{#1}}}
\else
\newcommand{\id}[1]{\ensuremath{1_{#1}}}
\fi

% Caligraphic category names
\newcommand{\catA}{\ensuremath{{\cal A}}\xspace}
\newcommand{\catB}{\ensuremath{{\cal B}}\xspace}
\newcommand{\catC}{\ensuremath{{\cal C}}\xspace}
\newcommand{\catD}{\ensuremath{{\cal D}}\xspace}
\newcommand{\catE}{\ensuremath{{\cal E}}\xspace}
\newcommand{\catF}{\ensuremath{{\cal F}}\xspace}
\newcommand{\catG}{\ensuremath{{\cal G}}\xspace}
\newcommand{\catH}{\ensuremath{{\cal H}}\xspace}
\newcommand{\catP}{\ensuremath{{\cal P}}\xspace}
\newcommand{\catQ}{\ensuremath{{\cal Q}}\xspace}

% Boldified names of useful categories (and some less useful!)
%
\newcommand{\vectfd}[1]{% category of f.d. vector spaces over some field
\ensuremath{\mathbf{Vect}^{\mathrm{fd}}_{#1}}\xspace}
\newcommand{\vectfdc}{% category of f.d. vector spaces over complexes
\vectfd{\mathbb{C}}}
\newcommand{\catRel}{% the category of sets and relations
\ensuremath{\mathbf{Rel}}\xspace}
\newcommand{\catSet}{% the category of sets and functions
\ensuremath{\mathbf{Set}}\xspace}
\newcommand{\catCat}{% the category of (small) categories
\ensuremath{\mathbf{Cat}}\xspace}
\newcommand{\catInvCat}{% the category of involutive categories
\ensuremath{\mathbf{InvCat}}\xspace}
\newcommand{\catComCl}{% the category of compact closed  categories
\ensuremath{\mathbf{ComCl}}\xspace}
\newcommand{\catSComCl}{% the category of strongly compact closed  categories
\ensuremath{\mathbf{SComCl}}\xspace}
\newcommand{\catGrph}{% the category of graphs
\ensuremath{\mathbf{Grph}}\xspace}
\newcommand{\qubit}{% the category of qubits
\ensuremath{\mathbf{Qubit}}\xspace}
\newcommand{\fdhilb}{% the category of finite dimensional hilbert space
\ensuremath{\mathbf{fdHilb}}\xspace}
\newcommand{\fdHilb}{\fdhilb}
\newcommand{\catInvCom}{% the category of involutive categories
\ensuremath{\mathbf{InvCom}}\xspace}
\newcommand{\catCom}{% the category of compact closed  categories
\ensuremath{\mathbf{Com}}\xspace}
\newcommand{\superop}{% the category of superoperators
\ensuremath{\mathbf{SuperOp}}\xspace}

\newcommand{\Set}{\catSet}
\newcommand{\Rel}{\catRel}
\newcommand{\Pfn}{% the category of partial functions
\ensuremath{\mathbf{Pfn}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% commutative diagrams
\usepackage{tikz-cd}
\newcommand{\lpushout}{\arrow[ur,phantom,"\urcorner",very near start]}
\newcommand{\rpushout}{\arrow[ul,phantom,"\ulcorner",very near start]}

%%%%%% nice idea doesn't work though.
%\newcommand{\inlinetikzcd}[1]{%
%\begin{tikzcd}[cramped, sep=small, ampersand replacement=\&] #1 \end{tikzcd}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% I use this pretty often...
\newcommand{\zxcalculus}{\textsc{zx}-calculus\xspace}
\newcommand{\zxdiagram}{\textsc{zx}-diagram\xspace}
\newcommand{\zxdiagrams}{\textsc{zx}-diagrams\xspace}
\newcommand{\ZX}{\ensuremath{\mathbf{ZX}}\xspace}
\newcommand{\ZXs}{\ensuremath{\mathbf{ZX_s}}\xspace}

\newcommand{\Enc}{\ensuremath{\mathrm{Enc}}\xspace}
\newcommand{\Dec}{\ensuremath{\mathrm{Dec}}\xspace}

%%%%%%%% useful names for Cliffords

\usepackage{dsfont}
\newcommand{\ID}{\mathds{1}}

\newcommand{\Cliff}{\ensuremath{\mathbf{Cliff}}\xspace}

\newcommand{\C}[1]{%
\ensuremath{\mathcal{C}_{#1}\xspace}}

% \newcommand{\CC}[1]{%
% \ensuremath{\mathfrak{C}_{#1}\xspace}}
\newcommand{\CC}{%
\ensuremath{\mathcal{C}}\xspace}   

\renewcommand{\P}[1]{%
\ensuremath{\mathcal{P}_{#1}\xspace}}

\newcommand{\eq}{\ensuremath{\stackrel{*}{\leftrightarrow}}}
\newcommand{\eqqq}{\ensuremath{\stackrel{*}{\longleftrightarrow}}}
\newcommand{\rw}{\ensuremath{\stackrel{*}{\rightarrow}}}



\newcommand{\tket}{\ensuremath{\mathsf{t}|\mathsf{ket}\rangle}\xspace}


%%%%%%%% 

\DeclareMathOperator{\List}{\mathsf{List}}%
\DeclareMathOperator{\cList}{\mathsf{CList}}%
\renewcommand{\int}[1]{\ensuremath{\mathrm{int}(#1)}}


\newcommand{\IN}{\ensuremath{\mathsf{in}}\xspace}
\newcommand{\OUT}{\ensuremath{\mathsf{out}}\xspace}
\newcommand{\END}{\ensuremath{\mathsf{end}}\xspace}
\newcommand{\INC}{\ensuremath{\mathsf{inc}}\xspace}
\newcommand{\LAB}{\ensuremath{\mathsf{lab}}\xspace}
\newcommand{\PP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\OG}{\ensuremath{\mathbf{OG}}\xspace}
\newcommand{\OPG}{\ensuremath{\mathbf{Plane}}\xspace}
\newcommand{\VAR}{\ensuremath{\mathbf{Var}}\xspace}



%%-----------------------------------------------------
%% TODO HERE --- TIKZ STUFF
%%-----------------------------------------------------

%\usepackage{pdflscape} % used to get somethings sideways


%%-----------------------------------------------------
%% MISC PACKAGES
%%-----------------------------------------------------

\usepackage{subcaption}
\usepackage{csvsimple}
\usepackage{multirow}
\usepackage{makecell}

%%%% hyperref wants to be last
\usepackage{hyperref}

\usepackage{float} % Add this in your preamble
\usepackage{siunitx}  % Ensure better number alignment
\usepackage{booktabs} % Better table styling
\usepackage{colortbl} % For coloring cells
\usepackage{placeins}
\usepackage{xcolor}

